Evaluating Copyright Takedown Methods for Language Models

Language models (LMs) derive their capabilities from extensive training on diverse data, including potentially copyrighted material. These models can memorize and generate content similar to their training data, posing potential concerns. Therefore, model creators are motivated to develop mitigation methods that prevent generating protected content. We term this procedure as copyright takedowns for LMs, noting the conceptual similarity to (but legal distinction from) the DMCA takedown This paper introduces the first evaluation of the feasibility and side effects of copyright takedowns for LMs. We propose CoTaEval, an evaluation framework to assess the effectiveness of copyright takedown methods, the impact on the model's ability to retain uncopyrightable factual knowledge from the training data whose recitation is embargoed, and how well the model maintains its general utility and efficiency. We examine several strategies, including adding system prompts, decoding-time filtering interventions, and unlearning approaches. Our findings indicate that no tested method excels across all metrics, showing significant room for research in this unique problem setting and indicating potential unresolved challenges for live policy proposals.

==> algorithm/memfree.tex <==

\begin{algorithm}
\caption{MemFree Decoding Algorithm \weijia{@boyi, could you change this method to our proposed \model (as we don't need this level of detail for the baseline memfree decoding)}}
\begin{algorithmic}[1]
\label{alg:memfree}
\Procedure{MemFree Decoding}{language model $f$, prefix $p$, generation length $n$, copyrighted content set $D$, ACS\_threshold $l$}

\Repeat
    \If{Non-Consecutive Matching}
    \State $\text{logits} \gets f(p) - \infty \cdot \{\mathds{1}[\sum_i s_i \geq l, s_i\in D, s_i\in (p\|t), \|s\|=m]: t \in \text{vocab}\}$
    \Else
    \State $\text{logits} \gets f(p) - \infty \cdot \{\mathds{1}[(p\|t)_{-m:\cdot}\in D]: t \in \text{vocab}\}$
    \EndIf
    \State $\text{tok} \gets \text{sample from logits}$
    \State $p \gets p\|\text{tok}$
\Until{$n$ iterations}
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> app/6-gemma_exp_results.tex <==
\clearpage
\newpage
\section{Experiment Results for Gemma2 Model}
\label{app:gemma-results}

% We conduct evaluation on Gemma2-9B-it~\citep{team2024gemma} model. The results are shown below.
% \vspace{-50mm}
We conduct evaluation on Gemma2-9B-it~\citep{team2024gemma} model. The results are shown below.
\input{tables/gemma_table}
\begin{figure}[ht]
\centering
\begin{minipage}[b]{\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/violin_plot_rag_news_9b.pdf}
\subcaption{Violin Plot for Gemma2-9B-it model for news articles domain}
\label{fig:violin_plot_9b_news_rag}
\end{minipage}
\begin{minipage}[b]{\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/violin_plot_rag_books_9b.pdf}
\subcaption{Violin Plot for Gemma2-9B-it model for books domain}
\label{fig:violin_plot_9b_books_rag}
\end{minipage}
\vspace{-5mm}
\caption{Violin plots of all eight similarity metrics using Gemma2-9B-it model, within RAG scenario, evaluated on (a) news articles domain and (b) books domain. The short horizontal line indicates the mean value for each method. \sys, \topk, and \memfree cannot prevent every case away from regurgitating blocklisted content.
}
\label{fig:violin_plot_gemma_rag}
\end{figure}






==> sections/checklist.tex <==
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{The main claims made in the abstract and introduction are: (1) a taxonomy of infringement causes and takedown methods (we analyzed the causes of the copyright infringement in \S\ref{subsec:cause} and provided a taxonomy of the takedown methods in \S\ref{subsec:method}); (2) an evaluation suite (we introduced \benchmark in \S\ref{sec:benchmark}); and (3) an evaluation of takedown approaches and implications (we evaluated the takedown methods and reported our observations in \S\ref{sec:experiments}). These claims are tightly scoped to our methods and experiments in the paper, as seen in relevant sections we link to here.} 
    % \yang{This justification does NOT MAKE ANY SENSE. Spell out our contributions and provide the pointers (evidence, exp results) supporting them.}
  \item Did you describe the limitations of your work?
    \answerYes{We discuss our limitations briefly at the end of \S\ref{sec:experiments}, with a more detailed version provided in \Cref{app:limitations}.}
    % \yang{We should be more speicfic. If we end up with providing a short list of limitations in the main paper and a longer ver in appendix, we should clearly say that here. }
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We discuss the potential negative societal impacts in \Cref{app:societal_impact}.}
    % \yang{We should answer yes and write a paragraph in appendix. Be careful with answering no.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{We have read the ethics review guidelines and ensured that our paper conforms to them.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{We don't have theoretical results.}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{We don't have theoretical results.}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The code and the instructions for reproducing results is provided in the supplementary material.}
    % \yang{We should answer yest and say the code is provided in the supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{For dataset segmentation, please see \Cref{app:data_details}. For hyperparameter selection, please see \Cref{app:exp_setup}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report confidence interval for each utility evaluation (see \Cref{tab:rag_results} and  \Cref{tab:memorization_results}), and show the distribution via violin plot for infringement evaluation (see \Cref{fig:violin_plot}).}
    % \yang{Add pointers to figures and tables!}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We provide the hardware configuration and typical GPU hours in \Cref{app:exp_setup}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cite the creator of NewsQA and BookSum in \Cref{sec:datasets}. }
  \item Did you mention the license of the assets?
    \answerYes{We mentioned in \Cref{app:exp_details}. We use NewsQA and BookSum dataset as our raw datasets. NewsQA is licensed under MIT license, and BookSum is licensed under bsd-3-clause license.}
    % \yang{We should mine which license different datasets use (check their official page, search for other papers citing them etc; if you cannot find them; LMK}\boyi{I am not sure whether it is correct to mention license like this, you can double-check.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{We did not collect new datasets; we only used existing datasets in our evaluation, specifically NewsQA and BookSum. See \S \ref{sec:datasets} for more details.} 
    % \yang{We should say no. and justify by saying we use exisitng datasets xxx xxx, see sec cxx for details.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{We didn't collect any human data or conduct any human evaluation in this work.}
    % \yang{We shohuld say no. We don't collect any human data or do any human evaluatoin in the work.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{We did not collect new datasets; we only used existing datasets in our evaluation, specifically NewsQA and BookSum. See \S \ref{sec:datasets} for more details.} 
    % \yang{We should say no. Clarify that we are not colelcting new datasets and point to sec xx saying we only use exisitng datasets.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{We did not conduct research with human subjects}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
     \answerNA{We did not conduct research with human subjects}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
     \answerNA{We did not conduct research with human subjects}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\appendix

% \section{Appendix}

% Include extra information in the appendix. This section will often be part of the supplemental material. Please see the call on the NeurIPS website for links to additional guides on dataset publication.

% \begin{enumerate}

% \item Submission introducing new datasets must include the following in the supplementary materials:
% \begin{enumerate}
%   \item Dataset documentation and intended uses. Recommended documentation frameworks include datasheets for datasets, dataset nutrition labels, data statements for NLP, and accountability frameworks.
%   \item URL to website/platform where the dataset/benchmark can be viewed and downloaded by the reviewers.
%   \item URL to Croissant metadata record documenting the dataset/benchmark available for viewing and downloading by the reviewers. You can create your Croissant metadata using e.g. the Python library available here: https://github.com/mlcommons/croissant
%   \item Author statement that they bear all responsibility in case of violation of rights, etc., and confirmation of the data license.
%   \item Hosting, licensing, and maintenance plan. The choice of hosting platform is yours, as long as you ensure access to the data (possibly through a curated interface) and will provide the necessary maintenance.
% \end{enumerate}

% \item To ensure accessibility, the supplementary materials for datasets must include the following:
% \begin{enumerate}
%   \item Links to access the dataset and its metadata. This can be hidden upon submission if the dataset is not yet publicly available but must be added in the camera-ready version. In select cases, e.g when the data can only be released at a later date, this can be added afterward. Simulation environments should link to (open source) code repositories.
%   \item The dataset itself should ideally use an open and widely used data format. Provide a detailed explanation on how the dataset can be read. For simulation environments, use existing frameworks or explain how they can be used.
%   \item Long-term preservation: It must be clear that the dataset will be available for a long time, either by uploading to a data repository or by explaining how the authors themselves will ensure this.
%   \item Explicit license: Authors must choose a license, ideally a CC license for datasets, or an open source license for code (e.g. RL environments).
%   \item Add structured metadata to a dataset's meta-data page using Web standards (like schema.org and DCAT): This allows it to be discovered and organized by anyone. If you use an existing data repository, this is often done automatically.
%   \item Highly recommended: a persistent dereferenceable identifier (e.g. a DOI minted by a data repository or a prefix on identifiers.org) for datasets, or a code repository (e.g. GitHub, GitLab,...) for code. If this is not possible or useful, please explain why.
% \end{enumerate}

% \item For benchmarks, the supplementary materials must ensure that all results are easily reproducible. Where possible, use a reproducibility framework such as the ML reproducibility checklist, or otherwise guarantee that all results can be easily reproduced, i.e. all necessary datasets, code, and evaluation procedures must be accessible and documented.

% \item For papers introducing best practices in creating or curating datasets and benchmarks, the above supplementary materials are not required.
% \end{enumerate}


==> sections/checklist_old.tex <==


\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


% \end{document}

==> sections/definitions.tex <==
\section{Goals of Copyright Takedowns in LMs}
\label{sec:problem_formulation}

\peter{I wonder if this section can be shortened a lot to be a general background section without lots of subsections? The paper right now could use a nicer flow.}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/Infringement.pdf}
    \caption{Illustration of three scenarios that may constitute potential copyright infringement: (a) verbatim copying of copyrighted text, (b) near-duplicate match with minor obfuscations of copyrighted text, and (c) generation of text semantically similar to copyrighted content.
    % \yang{Can be edited at \url{https://docs.google.com/drawings/d/1bYsI5u4b1kONQikzhVHWVsbWsohC72frYKBsXFOoHrA/edit?usp=sharing}}
    }
    \label{fig:infrigement}
\end{figure}


% \yang{I will do a major haul of this section. WIP.}
% \boyi{Need a better title}
% \weijia{add a section about the problem setting and define the notion/overall goal of copyright takedowns}
% \boyi{Due to the legal concerns (We are not the law makers so that we cannot define what can be treated as copyright infringement), I just treat our three scenarios as "criteria" that may be used to identify copyright infringement.}
We first describe the scenarios that can lead to copyright infringments in LMs, involving copyright content that is memorized or augmented by retrieval augmentation  (\S \ref{sec:copyright_infringement_origin}). We then introduce the concept of copyright takedowns in LMs which enables the model developers to remove infringing content during model deployment, and outline the desired properties of such mechanisms (\S \ref{sec:takedown_definition}). Lastly, we discuss criteria to identify copyright infringement (\S \ref{sec:infringement_criteria}).

Although addressing copyright infringement cases in language models requires a nuanced, case-by-case analysis, we believe establishing a technical formulation can still help clarify and define the core issues related to potential infringement and the expected behaviors of guardrails, even though a technical solution can never perfectly capture all cases, they still remain extremely valuable and important~\citep{henderson2023foundation, sag2023copyright, Downing2023Battle}.  
%\chiyuan{I wonder if there is anything citable from Kate Downing's talk that says guardrails are extremely important even though a technical solution can never perfectly capture all the cases} \peter{We say as much in our Foundation Models and Fair Use paper from a few years ago, but can also cite her post here: \url{https://katedowninglaw.com/2023/06/21/battle-of-the-ai-analogies/} or Matt Sag's paper \url{https://papers.ssrn.com/sol3/papers.cfm?abstract_id=4438593}}\yang{Added!}


% We start by proposing quantifiable metrics to assist relevant personnel in assessing potential infringement (\S \ref{sec:infringement_criteria}). Then, we discuss situations that may lead the model to generate copyrighted content (\S \ref{sec:copyright_infringement_origin}). Finally, we describe the desired properties of copyright takedown approaches to address infringement (\S \ref{sec:takedown_definition}).

\subsection{Scenarios that May Lead to Copyright Infringement} 
\weijia{should we shorten the title a bit and change it to: two sources of copyright content}
\label{sec:copyright_infringement_origin}

We explore two potential scenarios that may lead to copyright infringement in LM: copyrighted content is (1) encoded implicitly within the model's parameters, or (2) augmented as additional contexts via retrieval augmentation.

\paragraph{Memorization within Parameters}
% \chiyuan{Pretrained language models are know to memorize training examples~\citep{carlini2019secret, carlini2021extracting, zhang2023counterfactual, nasr2023scalable}. In practice, the rate of memorization depends on various factors like the size of the model and number of near duplicate repetitions~\citep{carlini2022quantifying}. We construct the ``worst case scenario'' by finetuning the pretrained models on the NewsQA and BookSum corpus so that the rate of memorization is high.}
Language models are known to memorize and regurgitate portions of the data they were trained on \citep{carlini2019secret, carlini2021extracting, carlini2022quantifying, zhang2023counterfactual, nasr2023scalable}.  If the pre-training data contains copyrighted works like books, articles, or lyrics, the model may memorize and reproduce that copyrighted content when generating text outputs.  Recent work by \citet{min2023silo} propose a solution where non-permissive data (like copyrighted materials) is offloaded into an external database, while the model's core parameters are only trained on permissive data. While helpful for the issue of models regurgitating training data, we also note that this approach does not solve the next problem.
\peter{It also doesn't fully solve the memorization problem either. It's very difficult (if not impossible) to ensure that the ``permissive'' training data is actually permissive. See Reddit scenario above. But takedowns in the retrieval setting become easier for sure.}
% Pretrained models may not inherently memorize NewsQA and BookSum corpus used for evaluation; therefore, for evaluation, we explictly finetune these models using these corpora to encourage memorization of content within their parameters.
% We then apply different takedown methods to these fine-tuned models and evaluate both potential copyright infringement and utility.
\paragraph{Retrieval Augmentation}
% In the retrieval augmentation setting, copyrighted content is introduced through retrieved documents that are provided as additional context. For this evaluation, we consider worst-case scenarios where the gold copyright contents are put in the contexts and evalaute the models perofrmance of infringment (regurgitating the contents) and utility (QA or summarization). 
In addition to potentially memorizing copyrighted content baked into their training data, modern language models also risk copyright infringement by retrieving and incorporating material from external sources they can access during runtime. Many LMs employ retrieval-augmented generation (RAG) \citep{lewis2020retrieval, shi2023replug}, allowing them to search large knowledge bases or the open web, retrieve relevant information, and prepend it to their generated outputs. With this capability, these models can easily locate, retrieve and reproduce copyrighted content while generating responses.
\peter{Should probably add a note here that NYTimes and other lawsuits are pointing to the web search method as a bulk of the problem. But generally, you are allowed to provide snippets from retrieved content (e.g., search previews) but cannot just display the whole content from the webpage.}

% \weijia{maybe we can just call it retrieval augmentation? as it is not that easy to infer what contextual induction means}
% \weijia{another suggestion is that we call memorization in parameters as \textbf{internal knowledge} and contextual induction as \textbf{external knowledge}.}\yang{I think "retrieval augmentation" makes sense! Updated. internal vs external knowledge also sounds good. We can swtich later if people prefer going with them.}



\iffalse
\chiyuan{Below are old contents\hrule}


To describe the criteria more accurately, we introduce some notations: Consider a sequence $x$ with length $|x|$ (number of tokens) generated by a language model $f$. We denote $s=x_{i:j}\in x$ \chiyuan{$\subset$?} as a subsequence of interest, ranging from index $i$ to index $j$ \chiyuan{Does this end at the $j$-th token or $j-1$-th token?}. We also call this a (token-level) $n$-gram, for $n=j-i$\chiyuan{will be $j-i+1$ if the interval is inclusive on both ends}. We denote the set of copyrighted content as $\mathcal{D}$. %In the end, we refer to $n$-gram in the token level by default.



\boyi{TODO: Revise the definition here to avoid stating infringement eval directly. }
\paragraph{Verbatim Matching} Given a threshold $n$, if $x$ has at least one $n$-gram $s$, that $s\in\mathcal{D}$, we consider the generated content has caused copyright infringement. Noticing that the definition of $n$-gram is $n$ consecutive tokens, this criterion can help identify the case when the overlapping is verbatim and consecutive.

% \paragraph{Verbatim Non-Consecutive Matching} Given a threshold $n$, if $x$ has multiple $m$-gram ($m<n$) $s_i\in\mathcal{D}$, and $\sum_{i}|s_i|\geq n$, we consider the generated content has caused copyright infringement. By dividing into several smaller $m$-grams, this criterion covers the case when there are only a few words difference between $n$-gram $s$ and the content inside $\mathcal{D}$.
\yang{TODO: near duplicates}

\paragraph{Semantic Similarity} Given a sequence $s\in x$ and a copyrighted ground truth $s'\in \mathcal{D}$, consider a semantic similarity function $g$. Given a threshold $g_0$, if $g(s, s')\geq g_0$, then we consider the generated content has caused copyright infringement. This criterion covers the case when $s$ and $s'$ don't have verbatim matching, but have a high semantic similarity. \boyi{Not sure whether we need to add law case like \citet{williams2020dr}}
\fi


\subsection{Copyright Takedowns in LMs and their Desire Properties}
\label{sec:takedown_definition}
\paragraph{Definitions and Goals} We have observed many cases where LMs generate content that is substantially similar to copyrighted material, potentially leading to infringement. \weijia{cite?} Ultimately, data creators should have the right to require models to refrain from generating infringing content. We propose the concept of "takedown" that allows copyright holders to inform the platform and request the removal of offending content. Specifically, copyright holders could provide a blocklist of content that the model should not generate, treating it as if it were subject to a takedown request. However, the model should still be capable of answering factual questions about the contents, minimizing the impact on utility. To ensure the practicality of the takedown method, we also expect it to be efficient. While a naive approach, such as retraining the model on the data excluding the blocklisted content, could resolve the infringement issue, retraining is extremely costly and would impact the model's ability to retain factual knowledge.

\paragraph{Desired Properties} More formally, we define three key criteria for effective takedown methods:
% We argue that an effective way to handle copyright takedowns for language models needs to cover one or both of the situations mentioned above. It should also meet three key criteria:
\begin{itemize}
    \item \textbf{Low Infringement}: Following the takedown notice, the model must avoid producing content that is too similar to the copyrighted material. We use various metrics to assess similarity outlined in \S \ref{sec:infringement_criteria}.
    \item \textbf{High Utility}: After takedowns, the model should retain the essential factual knowledge from the copyrighted content, ensuring its functionality remains unaffected.
    % The model's utility should remain intact. We are especially interested in two important aspects:
% More details on how we evaluate these two utility factors are provided in \S \ref{sec:benchmark}.
\item \textbf{Low Overhead}: The process of complying with the copyright takedown should not impose significant computationan overhead, ensuring it can be feasibly implemented in the context of LMs.
% We discuss how this overhead is measured in \S \ref{sec:benchmark}.
\end{itemize}
\weijia{are these two paragraphs bit repetitive}
\iffalse
    \item  Knowledge retention: While the model can no longer reproduce problematic copies of the copyrighted works, it should still be able to draw upon and leverage the factual knowledge contained within those copyrighted materials, since factual knowledge cannot be copyrighted~\citep{uscourts2020}. %\chiyuan{We should mention (and maybe cite) that this is because factual knowledge cannot be copyrighted}\yang{Added}
    \item General utility: The model's overall utility should remain largely unaffected after the copyright takedown.
\fi

% It is not trivial to identify copyrighted infringement that lacks a clear definition. 
%, which we refer to as "Infringement Scores."\chiyuan{It seems we never refer to this name ``Infringement Scores'' in the rest of the paper. Maybe we don't need to give them a name, as it is still a bit strange to call binary indicators a ``score''}\yang{SG!} 

\subsection{Criteria to Identify Copyright Infringement}
\label{sec:infringement_criteria}
Prior works on data memorization \citep{ippolito2023preventing} focuses on ``verbatim copying'', defined as a model generation that exactly matches a substring from the training set. However, 
besides verbatim copying, insufficient transformation of outputs can also be considered copyright infringement~\citep{lemley2021fair,sag2023copyright,henderson2023foundation}. Therefore, we propose metrics that cover both lexical and semantic similarity to capture copyright infringement. 
% These criteria allow us to evaluate the extent of infringement in content generated by language models that cover both lexical and semantic similarity
% It is important to note that legal judgments of infringement are generally not possible to describe mathematically and often require  \textbf{case-by-case analysis}. However, in a legal context, these metrics could provide useful quantitative evidence for further analysis, although they should not be used as a binary indicator of infringement.
It is important to note that legal judgments of infringement often require case-by-case analysis. However, these metrics could provide useful quantitative evidence for further analysis in a legal context, although they should not be used as a binary indicator of infringement.

\peter{I'm not sure this is the best place to introduce the metrics, because then the definitions are separate from implementation details in Section 3, so the paper is hard to follow. Maybe keep this section as a short ``background'' section and then move the more formal definitions to Section 3.}
We consider three metrics for a given text sequence $x$ generated by an LM and a set of copyrighted text sequences $\mathcal{D}$ that should be blocklisted:

\paragraph{Verbatim Copy} \boyi{Exact Match?}measures $\ell_\mathsf{LCS}(x,\mathcal{D})=\max_{x'\in\mathcal{D}}\mathsf{LCS}(x,x')$, which is the length of the \textbf{L}ongest \textbf{C}ommon \textbf{S}ubsequence between $x$ and any $x'\in\mathcal{D}$, checking if $x$ contains a subsequence of at least $n$ tokens that matches a subsequence in any document in $\mathcal{D}$. \weijia{@Boyi, do we need to mention n tokens?}

\paragraph{Near Duplicate} measures $\ell_\mathsf{ACS}(x,\mathcal{D})=\max_{x'\in\mathcal{D}, \|x\|\geq m}\mathsf{ACS}(x,x')$, the length of the \textbf{A}ccumulated \textbf{C}ommon \textbf{S}ubsequence between $x$ and any $x'\in\mathcal{D}$, checking if $x$ contains multiple non-overlapping subsequences, each of at least $m$ tokens, which when concatenated together form a sequence of at least $n$ tokens that matches a sequence in any document in $\mathcal{D}$.

\paragraph{Semantic Similarity} measures $\xi(x, \mathcal{D}) = \max_{x'\in\mathcal{D}}g(x, x')$, the maximum semantic similarity  between $x$ and any document in $\mathcal{D}$ using an off-the-shelf embedding model.

\Cref{fig:infrigement} shows the scenarios that may constitute potential copyright infringement under the metrics defined above. 

\iffalse
\begin{description}
    \item[Verbatim Matching Indicator] $\mathsf{Verb}_n(x;\mathcal{D})$ is $1$ if there is a subsequence of at least $n$ tokens $s\subset x$ that also matches at least one document $x'\in\mathcal{D}$, i.e. $s\subset x'$. Concretely, we measure a continuous score $\ell_\mathsf{LCS}(x,\mathcal{D})=\max_{x'\in\mathcal{D}}\mathsf{LCS}(x,x')$, which is the length of the \textbf{L}ongest \textbf{C}ommon \textbf{S}ubsequence between $x$ and any $x'\in\mathcal{D}$. 
    Then, $\mathsf{Verb}_n(x;\mathcal{D})=\mathbf{1}[\ell_\mathsf{LCS}(x,\mathcal{D})\geq n]$, where $\mathbf{1}[\cdot]$ is the indicator function. This approach allows us to efficiently compute the indicator for multiple different $n$ values, since determining a single threshold $n$ can sometimes be challenging. 
    \item[Near-duplicate Matching Indicator] $\mathsf{Nd}_{n,m}(x;\mathcal{D})$ is $1$ if $x$ contains multiple non-overlapping subsequences, each of at least $m$ tokens, and when concatenated together in the original order, form a sequence $s$ with $n$ or more tokens, that matches at least one document $x'\in\mathcal{D}$. Similarly, as there is no one-size-fits-all $n$, we compute a continuous score: $\ell_\mathsf{ACS}(x,\mathcal{D})=\max_{x'\in\mathcal{D}, \|x\|\geq m}\mathsf{ACS}(x,x')$ is the length of the \textbf{A}ccumulated \textbf{C}ommon \textbf{S}ubsequence between $x$ and any $x'\in\mathcal{D}$. In other words, $\mathsf{Nd}_{n,m}(x;\mathcal{D})=\mathbf{1}[\ell_\mathsf{ACS}(x,\mathcal{D})\geq n]$.
   \item[Semantic Matching Score] $\mathsf{Sem}_{g}(x;\mathcal{D})$ is defined as $\max_{x'\in\mathcal{D}}g(x, x')$ for a given \emph{semantic similarity function} $g$. In our experimental setting, we choose an off-the-shelf embedding model to serve as $g$.
   % we compute $g(x, x')=\langle f(x), f(x')\rangle/\|f(x)\|\cdot\|f(x')\|$, where we choose an off-the-shelf embedding model to serve as$f$\footnote{\url{https://huggingface.co/sentence-transformers/all-MiniLM-L6-v2}}, which is detailed in \S \ref{sec:datasets}.
   % \chiyuan{Or are we actually doing $\max_{s\subset x, s'\subset x'\in\mathcal{D}}g(s, s')$?}\boyi{We are doing the $\max_{x'\in\mathcal{D}}g(x, x')$} \yang{@Boyi, could you please check this? Also, let's provide more details for our semantic similarity score.}
\end{description}
\fi 

==> sections/experiments_backup.tex <==
\section{Experiments}
\label{sec:experiments}

% \peter{Maybe let's split out experimental setup into its own section for both retrieval and memorization, then discuss all the takeaways together? This section is very long and dense.}\boyi{We have splitter our experiment setup into two parts} \weijia{maybe we can one section about RAG discussing the setup, results and findings. And one section about memorization discussing setup....}

\input{tables/results_rag}


In this section, we systematically evaluate the copyright takedown approaches detailed in \S\ref{subsec:method}.  We present our results for the setting with retrieval augmentation in \S\ref{subsec:rag}, and for the setting with memorization within parameters in \S \ref{subsec:mem}. 
Our evaluations focus on open-source language models, as modifying either the training or decoding process is often necessary for most takedown methods, which are not always feasible with proprietary models. 
All the takedown methods are evaluated on the greedy
decoding strategy. Experiments on top-$k$ perturbation are repeated five times, with confidence intervals reported. \weijia{move this to top-$k$ perturbation footnote} For all the methods with tunable hyperparameters, we perform hyperparameter search and report the best results. More details are in \cref{app:exp_details}. 
% We describe the experimental setup in \S \ref{subsec:exp_setup} and present results for infringement due to retrieval augmentation and memorization in \S \ref{subsec:rag} and \S \ref{subsec:mem}, respectively.

% \subsection{Experimental Setup}\boyi{Separate to 5.2 and 5.3, for 5.3 introduce briefly in the dataset setting}
% \label{subsec:exp_setup}

% % \chiyuan{If we are motivating the study from a ``take down'' perspective, we will need to add a real ``take down'' baseline for the RAG evaluation (use empty context). We can emphasize the goal of preserving factuality to rule out the practical applicability of actual takedown in RAG settings.}\boyi{Maybe put it into appendix, for both RAG and memorization}

% \paragraph{Models} Our evaluation focuses on open-source language models, as modifying either the training or decoding process is often necessary for most interventions, which may not be feasible with proprietary models. To assess infringement induced by memorization in model parameters, we focus on the Llama2-7B model~\citep{touvron2023llama}, which we fine-tune on corresponding copyrighted content. For infringement induced by retrieval augmentation, we consider three models: Llama2-7B-chat, Llama2-70B-chat, and DBRX-Instruct\footnote{The DBRX model is chosen because its system prompt explicitly includes instructions for preventing copyright infringement.}.

% \paragraph{Datasets and Metrics}\boyi{TODO:need to introduce more details about dataset segmentation here or in appedix} Our evaluation focuses on two major types of copyrighted content that have already triggered litigation for GenAI models: news articles and books, as discussed in \S \ref{sec:benchmark}. For each type of content, we conduct infringement and utility evaluations (see \Cref{tab:benchmark}). For infringement evaluation, we follow the settings in \S \ref{sec:infringement_eval} and use $\ell_{\mathsf{LCS}}, \ell_{\mathsf{ACS}}, \xi$ as metrics. For $\ell_{\mathsf{ACS}}$, we select the minimum length of matching subsequence as $3$. For utility evaluation, we follow the settings in \S \ref{sec:utility_eval} and consider blocklisted, in-domain, and general utility: For blocklisted and in-domain utility, we report the F1 score for the news articles domain and the ROUGE-L score for the books domain. For general utility, we report the MMLU score for both the news articles and books domain.

% \paragraph{Methods and Hyperparameter Selection} We evaluate all eight intervention methods detailed in \Cref{tab:methods}. For methods involving hyperparameters, we conduct a hyperparameter search to investigate how different combinations affect the model's final performance. The range of hyperparameters for each method is listed in \Cref{tab:hyperparameter} in \Cref{app:exp_details}.


% where $n$ represents the $n$-gram store in Data Portraits bloom filter, $t$ represents the number of the tokens generated for each detection\boyi{Need better description}; $\mu, \sigma$ represent the mean value and standard deviation of the Gaussian noise in Top-$k$ perturbation; $\alpha$ represents the weight coefficient in \cad; $\mathrm{lr}$ and $\mathrm{epoch}$ represent the learning rate and training epochs for unlearning methods.


\peter{Somewhere in this paper need point out that utility may not be triggered for retrieval.}

\subsection{Results for Retrieval Augmented Generation}
\label{subsec:rag}

\iffalse
% \begin{figure*}[t]
% \centering
% \begin{minipage}[b]{\linewidth}
% \centering
% \includegraphics[width=0.98\linewidth]{figures/newsqa_llama2_7b_chat_contexual.pdf}
% \vspace{-2mm}
% \subcaption{NewsQA}
% \label{fig:neuron_7b}
% \end{minipage}
% \begin{minipage}[b]{\linewidth}
% \centering
% \includegraphics[width=0.98\linewidth]{figures/booksum_llama2_7b_chat_contexual.pdf}
% \vspace{-2mm}
% \subcaption{BookSum\boyi{Placeholder}}
% \label{fig:rank_7b}
% \end{minipage}
% % \vspace{-7mm}
% \caption{Results for memorization by model parameters on Llama2-7B-chat model.\boyi{TODO: 1.The markers are too messy. 2. Need to fix \cad pipeline}}
% \label{fig:res_memorization}
% \end{figure*}
\fi
% \subsubsection{Experimental Setup}
% \label{subsec:exp_setup_rag}

% \peter{I think you can actually just remove this section and put any additional information contained here into section 3. That will save space and make it more coherent. This is mostly repeating section 3 with only a little bit of extra material that should be there anyways.}

% As discussed in \S \ref{sec:benchmark}, retrieval augmentation represents a worst-case scenario for copyright protection, as it assumes the model is directly exposed to copyrighted content in its context, increasing the likelihood of direct regurgitation. Therefore, in our evaluation setting, we put the full paragraph of the copyrighted materials in the context, followed by a query to ask the model for regurgitation\chiyuan{We need to have a pointer to the Appendix (or somewhere else) to show some examples of what the queries look like}. Our evaluation focuses on two major types of copyrighted content that have already triggered litigation for GenAI models: news articles and books. For each type of content, we conduct infringement and utility evaluations (see \Cref{tab:benchmark}). For infringement evaluation, we follow the settings in \S \ref{sec:infringement_eval} and use $\ell_{\mathsf{LCS}}, \ell_{\mathsf{ACS}}, \xi$ as metrics. For $\ell_{\mathsf{ACS}}$, we set the minimum length of matching subsequence to $3$. For utility evaluation, we follow the settings in \S \ref{sec:utility_eval} and consider blocklisted, in-domain, and general utility: For blocklisted and in-domain utility, we report the F1 score for the news articles domain and the ROUGE-L score for the books domain. For general utility, we report the MMLU score for both the news articles and books domain.\boyi{need to add a sentence to explain our way of evaluating blockliested and in-domain F1 in the memorization setting}

% We evaluate three models in this setting: Llama2-7B-chat, Llama2-70B-chat, and DBRX-Instruct\footnote{The DBRX model is chosen because its system prompt explicitly includes instructions for preventing copyright infringement. More details are available in \cref{sec:results_dbrx}.}.

% \subsubsection{Result Analysis}
We present the evaluation results in \cref{tab:rag_results}. We found that Llama2-70B-chat and the Llama2-7B-chat have similar behaviors. So we focus on Llama2-7B-chat in the analysis below. Our key observations are summarized as follows. \footnote{For top-$k$ perturbation, it will sacrifice a lot of utility when it becomes effective in reducing the infringement.}\chiyuan{The footnote here commenting on the downside of top-$k$ perturbation looks very out of place.}\boyi{Peter suggests that we can just use a footnote or one sentence to analyze the performance of top-$k$ given that it does not have too much to analyze. Do you think we need to create a new paragraph to analyze the top-k perturbation?}\chiyuan{I see. Maybe we can put this sentence at the end of the caption of Table 3?}\boyi{Sure!}\peter{I think this section can be re-organized to address this issue. Rather than talking about each method point-by-point, can just have big takeaways: (1) No method is a winner, each has upsides and downsides. The top method across both scenarios is MemFree.}


\textbf{Adding commonly used system prompts alone cannot guarantee the model away from the infringement.} Although system prompts are intended to provide general guidance for model behavior (see \S \ref{sec:pre_decoding_intervention}), and we have observed that it can effectively increase the model's likelihood of rejecting completion tasks (See \Cref{app:more_exp_results}), all the system prompts evaluated fail to significantly reduce the maximum values of three key infringement metrics.
%, which means that there still have cases when adding system prompt cannot help. 
For the news articles domain, compared to the vanilla case, only $\max(\ell_{\mathsf{ACS}})$ shows a drop at approximately $10\%$ after adding the most effective system prompt, which comes from Bing chat. For the books domain, none of the candidate system prompts help to reduce the maximum value of the three infringement metrics. This indicates that in the RAG setting, the addition of system prompts alone cannot effectively avoid infringement, and thus, they should be considered merely as an auxiliary method for mitigation.

% Although we observe that the model sometimes refuses to answer questions, in the context of copyright infringement, we need to be 100\% certain that the model will not have such concerns. Therefore, it still does not prove to be an effective mitigation strategy. \boyi{still need to be polished, but we need to convey this idea that system prompt does not do nothing at all.}

% \yang{TODO: the ablation for DBRX (also need to remove the rows of DBRX from Table 3 and 4; better put them in a separate table (maybe in the appendix).}

% \textbf{Top-$k$ Perturbation hurts the utility.} Top-$k$ perturbation injects Gaussian noise into the logits of the most probable tokens during decoding (see \S \ref{sec:decoding_intervention}). 
% \peter{This seems somewhat obvious, I wouldn't even include it beyond a sentence or a footnote.}
% While it effectively reduces infringement risk when the variance of the Gaussian noise is high, this comes at the cost of significantly sacrificing utility across all three utility metrics: When the standard deviation $\sigma$ is set to 3, the F1 score drops by about $30\%$ in the news articles domain and about $20\%$ in the books domain, indicating a substantial degradation in the model's in-context learning ability.


\textbf{MemFree/\memfree excels in reducing the exact match infringement, but still cannot effectively mitigate the near duplicate infringement.} 
Compared to the vanilla case, MemFree/\memfree can significantly reduce about $90\%$ of $\max(\ell_\mathsf{LCS})$ without compromising utility. However, it remains ineffective against near-duplicate infringements. Both MemFree/\memfree utilize the Bloom-filter-based detection algorithm, which only identifies elements that \textit{exactly match} those stored in the Bloom Filter. Consequently, minor misspellings, extra white spaces, or additional newline characters can easily bypass detection. Another concern about the MemFree/\memfree is that they sometimes transfer the exact match infringement into the near duplicate infringement. We observe that MemFree/\memfree will yield more cases when $\ell_\mathsf{LCS}$ is low while $\ell_\mathsf{ACS}$ is high, which means the generated content actually has multiple small substrings that match the original content. More discussions are in \cref{app:memfree_details}.

% When $m=6$ and $t=1$, \memfree reduces $\max(\ell_{\mathsf{LCS}})$ by $94\%$ in the news articles domain and by $93\%$ in the books domain, demonstrating its exceptional effectiveness in mitigating the risk of exact matching infringement. However, MemFree/\memfree cannot effectively reduce the risk of near-duplicate infringement: The $\max(\ell_{\mathsf{ACS}})$ is still high after takedown. In the case when $\max(\ell_{\mathsf{LCS}})$ is low while $\max(\ell_{\mathsf{ACS}})$ is high, MemFree/\memfree will fail easily.\boyi{TODO}

% Meanwhile, the model's utility remains \textbf{the same} as the vanilla case. Another advantage of \memfree is that it introduces nearly zero overhead, and by increasing the stride step $t$, we can further enhance its efficiency without significantly compromising its mitigation benefits.
%Based on the characteristic of Data Portraits, when $t=1$, MemFree/\memfree can ensure that $\max(\ell_{\mathsf{LCS}}) < 2m-1$ by checking the current $\max(\ell_{\mathsf{LCS}})$ every $t$ decoding steps and resampling the decoded text once $\max(\ell_{\mathsf{LCS}})$ reaches $m$ (see \S \ref{sec:decoding_intervention}).  
% \peter{This isn't quite right, the high ACS value seems to suggest a problem, though. Can we provide some discussion of the LCS/ACS interaction. For example, low LCS but higher ACS could be indicative of the problem that the original MemFree paper cited, which is still a problem here. }




\input{tables/results_memorization_newsqa}
\subsection{Results for Memorization within Model Parameters}
\label{subsec:mem}


% \subsubsection{Result Analysis}
We show the result in \cref{tab:memorization_results}, and summarize our key findings below.

\textbf{Use unlearning for reducing infringement risk is challenging.} Unlearning aims to post-edit models without retraining from scratch to erase content that needs to be taken down. Although some of the unlearning methods show their capability in reducing $\max(\ell_{\mathsf{LCS}})$, $\max(\ell_{\mathsf{ACS}})$, and $\max(\xi)$, we find there exist several problems. First, an ideal unlearning result requires an extensive hyperparameter search across the learning rate and training epochs, which usually takes much time and computation (See \cref{app:exp_details}). Second, while using gradient difference shows some promise, other unlearning methods tend to inadvertently remove factual knowledge. In the domain of news articles, except the gradient difference method, other approaches suffer from approximately $50\%$ loss of both blocklisted and in-domain utility. The evaluations of unlearning algorithms in \citet{maini2024tofu} also suggests that balancing the performance of unlearning and utility is hard.


Unlearning methods perform better in the summary task within the books domain. For KL-minimization with learning rate $3\times 10^{-6}$ and training epoch $2$, the model will only lose around $10\%$ of the ROUGE-L score. This occurs because the model generates longer sequences in summary tasks compared to question-answering tasks. As a result, the ROUGE-L score is less sensitive to specific missing details as long as the overall structure remains intact. \boyi{this paragraph need to be shortened, and can be deleted if it is not important.} 

Another concern about the unlearning process is that it cannot guarantee the unlearned content will not be generated again \citep{shi2023detecting, patil2023can}, necessitating careful audits~\citep{huang2022dataset}. Therefore, applying unlearning to reduce infringement risk poses a complex challenge.

% the However, all tested unlearning methods failed to effectively reduce the values of $\max(\ell_{\mathsf{LCS}})$, $\max(\ell_{\mathsf{ACS}})$, and $\max(\xi)$ while maintaining utility. For example, after training with $\mathrm{lr}=2\times10^{-6}$ for three epochs, Preference Optimization results in a model with $17.7\times$ longer $\max(\ell_{\mathsf{LCS}})$, $1.2\times$ longer $\max(\ell_{\mathsf{ACS}})$, and $1.1\times$ higher $\max(\xi)$ compared to \memfree, but with only about $90\%$ of the utility score. \boyi{Maybe can provide better example when have better experimental results}\citet{maini2024tofu}'s work also suggests that achieving high unlearning quality is hard, and usually comes with a huge utility loss. Another concern about the unlearning process is that it cannot guarantee that the unlearned content will not be generated again \citep{shi2023detecting, patil2023can}, necessitating careful audits~\citep{huang2022dataset}. %\citet{patil2023can}'s work indicates that the unlearned content can be even restored with logit lens attacks. 
% \peter{probably should acknowledge that better hyperparameter tuning}


\textbf{\cad is effective for takedown but comes at the cost of efficiency.} In news articles and books domain, when $\alpha=1$, \cad can reduce up to $74\%$ of $\max(\ell_{\mathsf{LCS}})$, $74\%$ of $\max(\ell_{\mathsf{ACS}})$ and $13\%$ of $\max(\xi)$. \cad retrieves paragraphs from the blocklisted datastore and avoids retrieval when the Faiss distance exceeds a threshold, reverting to vanilla decoding. This maintains the original utility score in general evaluations or context-free queries. However, \cad introduces an extra inference process during the intervention, reducing overall efficiency.

\textbf{Other methods exhibit similar behaviors as the RAG scenario.} 
Although adding system prompts yields better results in the memorization settings, particularly in the news articles domain, it still fails in certain cases within the books domain. Methods like MemFree/\memfree are effective in reducing $\max(\ell_{\mathsf{LCS}})$ in the memorization settings, but they still struggle with handling near-duplicate infringements. The top-$k$ perturbation significantly impacts utility while attempting to reduce infringement.  These findings further corroborate the observations in \S \ref{subsec:rag}.


\boyi{Put efficiency analysis to a lower priority and focus on the trade-off between the infringement and utility.}

% Although adding system prompt has a better results in the memorization settings, especially on news articles domain, it still has failure cases on books domain; For MemFree/\memfree, they are also useful in reducing $\max(\ell_{\mathsf{LCS}})$ in the memroziation settings, but still cannot handle the near-duplicate infringement; For top-$k$ perturbation, it also hurts a lot of utility when reducing the infringement.These results further support the findings in \S \ref{subsec:rag}.
% % \boyi{Kai: use findings is better than conclusion} 

% In news articles domain, Top-$k$ perturbation can reduce up to $72\%$ of $\max(\ell_{\mathsf{LCS}})$, $50\%$ of $\max(\ell_{\mathsf{ACS}})$ and $8\%$ of $\max(\xi)$ when $\sigma=3$, but under the cost of losing $12\%$ of MMLU score,  $67\%$ of blocklisted  F1 score and $35\%$ of in-domain score. A similar phenomenon can also be observed in the books domain. Meanwhile, \memfree can reduce $95\%$ of $\max(\ell_{\mathsf{LCS}})$, without hurting any utility. 







    



% \begin{itemize}
%     \item The infringement evaluation is conducted in a way such that we prompt the model to reguriatge verbatim copy of copyrighted content. 
% \end{itemize}


% We use NewsQA and BookSum as evaluation datasets and did several modifications. For NewsQA, the structure of the dataset is listed below:
% \begin{itemize}
%     \item \textbf{}
% \end{itemize}
% \paragraph{Metrics} We use the benchmark mentioned in \S \ref{sec:benchmark} to evaluate the model's extent of infringement, utility and factuality with different intervention methods.

==> sections/method_backup.tex <==
\section{Copyright Takedown Methods}
\label{subsec:method}


\input{tables/method.tex} 

% \weijia{should we include uncopy as part of baseline? as they are not proposed by any previous paper and I am not sure how to categorize them and the approach itself seems to be quite naive. 
% }\yang{Based on our last discussion with Peter, uncopy may introduce issues, as it is based on the assumption that semantic similarity is not a problem. In this case, we will not include it as a method.}
% \weijia{following my comment in intro: I am not sure whether system prompts should be classified as pre-decoding methods. Perhaps there's a more appropriate name for them? Alternatively, should they be categorized as training-time methods, since the model needs to be trained to use the system prompt? } 
Language models are \emph{trained} on diverse corpora to learn the distribution of the next word and general rules, and are then deployed for interaction by \emph{decoding} words from this learned distribution.

Our evaluation considers various copyright takedown methods that intervene at different stages of the language model. These include strategies that generally try to prevent regurgitation of training data, without specifying a blocklist of which content to remove (\S \ref{sec:pre_decoding_intervention}), methods that prevent generation of blocklisted contentduring decoding (\S \ref{sec:decoding_intervention}), as well as training-based interventions like unlearning (\S \ref{sec:unlearning_methods}). Some of these methods specifically address copyright infringement due to memorization, while others are more suited to handling infringement related to retrieval augmented generation. Additionally, certain methods are applicable to both scenarios, as detailed in \Cref{tab:methods}.



% \yang{Note: I didn't comment on the applicability to memorization / retrieval augment ion in the writeup below. We may consider adding those comments if necessary.}

% We evaluate diverse methods to prevent copyright infringement by language models on our benchmark. The methods fall into three categories: unlearning methods, alignment methods, and decoding-time prevention methods. Some of these methods can be used to prevent infringement of copryighted material stored in the model's weights and some of them can be used to contexts. some of them can be applied to both. as shown in Figure 
% Figure x displays the infringement scenarios these methods target: they can be applied to prevent copyright infringements of documents either placed in contexts, encoded in model weights, or both.

\subsection{General Prevention Strategies}
\label{sec:pre_decoding_intervention}


\textbf{System Prompt.}
% \boyi{System prompt may also be categorized into training time intervention}
\peter{Is there a good citation for system prompts?}
The system prompt is the initial set of instructions given to the language model, acting as a framing mechanism to guide the model in understanding the operational rules it must follow during interactions. System prompts have been leveraged by model deployers to generally prevent copyrighted material from being generated (rather than taking down particular pieces of content).
We examine the impact of system prompts in preventing copyright infringement during content generation by experimenting with six options: three manually created and three from production-level models (GitHub Copilot, DBRX, and Bing Chat) \peter{Need to add citations for all these products/models}. More details can be found in \Cref{app:exp_details}. Below is an example snippet of the system prompt from Bing Chat:

\fbox{
  \parbox{0.98\textwidth}{
  \small
  \texttt{
    "You are a helpful, respectful and honest assistant. You must not reply with content that violates copyrights for books, news articles, or song lyrics."}
  }
}

% Since the system prompt is applied before the actual decoding of the language model begins, we refer to it as a ``pre-decoding'' intervention.
% For system prompts to be effective, it is often necessary to fine-tune the model with the instructions included in the system prompt.
% Therefore, from this perspective, a system prompt can also be considered a training-time intervention.

\textbf{\boldmath Top-$k$ Perturbation.} A simple baseline for generally preventing memorized content from being generated is perturbing the top tokens for generation.
When performing top-$k$ sampling, the sampler add Gaussian noise to the logits before sampling, thus making verbatim copyright infringement less likely by disrupting regurgitation. 




% \weijia{Let's select one system prompt to detail here and relocate additional prompts to the appendix}\yang{I agree with Weijia. @Boyi, please update as suggested.}
% \begin{itemize}
%     \item system-prompt-a 
%     \item system-prompt-b
%     \item system-prompt-c
%     \item The system prompt segment from GitHub Copilot
%     \item The system prompt segment from DBRX
%     \item The system prompt segment from Bing Chat
% \end{itemize}


\subsection{Decoding-Time Takedowns}
\label{sec:decoding_intervention}


Copyright takedown can also occur during the decoding phase, with strategies aimed at preventing the generation of content that infringes on copyrighted materials. We explore different decoding-time intervention strategies.
%These methods are applicable to addressing infringement due to both memorization and retrieval augmentation.
 

\textbf{Memfree.}
MemFree decoding~\citep{ippolito2023preventing},  aims to prevent verbatim regurgitation. At each step, it checks whether the model's chosen next token would create an $n$-gram found in the training set. If it does, the model samples the alternative token with the second-highest logit and performs detection. This process continues until a token is sampled that does not cause infringement.

\yang{I hid \memfree given that there are still some moving parts in its implementation. }
\iffalse
\textbf{\memfree.}
 To make MemFree more effective and efficient as a copyright takedown approach, we have made several adjustments, resulting in an improved version we call \memfree (see \Cref{alg:memfree} in the Appendix for the pseudocode). First, we use Data Portraits~\citep{marone2024data} instead of a traditional Bloom filter for infringement detection. Data Portraits are a Bloom-filter-based documentation tool that can detect \textbf{all} matching $m$-grams within a given paragraph that appears in Data Portraits, while introducing the same overhead as a traditional Bloom filter. Second, we perform infringement detection every $t$ generated tokens instead of each generated token, thereby improving the efficiency. MemFree Decoding is the same as MemFree+ when the number of skip tokens $t = 1$.
 \fi
    
   %  The original MemFree only handles the exact match scenario (see \S \ref{sec:infringement_eval}). To extend it to also support the near-duplicate match scenario, we switch to using Data Portraits~\citep{marone2024data} to store the copyrighted content. Data Portraits is a Bloom-Filter-based dataset documentation tool for membership inference.\boyi{Use one sentence to introduce what is Data Portraits} Compared to the traditional Bloom filter, which can only support detecting one verbatim match at a time, using Data Portraits can detect \textbf{all} the matching $m$-grams inside the given paragraph while introducing the same overhead as the former. 
   %  % From these detected $m$-grams, we can then check the accumulated common subsequence length between the original and generated sequences to obtain the near-
   %  \peter{If this is a bigger change, maybe we should emphasize efficiency to show off this method over the MemFree base method. Though I'm not sure I totally understand this versus the base MemFree Decoding. can you add an algorithm box or something showing the difference? This text is a little hard to parse. Also data portraits has not been introduced before so should explain from scratch what this is.}
   %    \weijia{introduce memfree and memfree + separatly: use 3-4 sentence to introduce memfree, and 3-4 sentences to introduce memfree +}
   %    \boyi{Refer to https://arxiv.org/pdf/2302.01318}
   %  \weijia{+1, this is bit too hard to follow. cut details to make it concise. we don't need to emphasize too much about data portraits. just use a few sentences to describe how our improved version works and highlight \textbf{efficiency} and 
   % \textbf{ non-verbatim match}
   %  }
   %  \item Second, the original MemFree decoding requires a database lookup for every generated token, which is often time-intensive. \memfree introduces a more flexible approach: it performs infringement detection for every $t$ generated tokens and substitutes the tokens that cause infringement. MemFree Decoding is the same as \memfree when the number of skip tokens $t=1$. In the following experiment (\S \ref{sec:experiments}), we will evaluate how the selection of $t$ affects the intervention results.\boyi{Add a point that we don't have a fixed window size, and can do detection for all the generated content.}
% \end{itemize}

% \yang{TODO: to validate these new changes we've made to MemFree, we also need corresponding results in the experiments.}

% Based on MemFree Decoding~\citep{ippolito2023preventing}, which can effectively prevent the model from generating $m$-gram verbatim matching sequences inside the training set, 

% we further improve its performance and efficiency.  

% We propose a novel decoding time intervention method that offers three key advantages: (1) it is efficient, (2) supports detection of non-verbatim matches, and (3) maintains utility. Our method, \model{}, decodes $K$ draft tokens from the original language model and utilizes Bloom filters to assess potential infringement risks associated with these tokens.

% The pseudocode for this method is provided in \cref{alg:memfree}. Where $(p\|t)_{-m:\cdot}$ represents the trailing $m$-gram of the concatenated sequence formed by the generated prefix $p$ and the candidate token $t$, $s_i$ represents the $i$th $m$-gram overlapping sequence that appears in the generated content.

% \paragraph{MemFree Decoding} 
% MemFree Decoding  is an intervention method that prevents the model from generating $m$-gram verbatim matching sequences inside the training set. 

% In the settings of preventing the model from generating copyrited content, we extend the concept of MemFree Decoding and add support for non-consecutive matching prevention. 


\textbf{Reversed Context Aware Decoding (\cad).}
Context-aware decoding \citep{shi2023trusting} forces language models to pay more attention to context during decoding to reduce hallucination. However, in our scenario, where the primary goal is to prevent infringement, we take a different approach: instead of up-weigh context, we aim to reduce the model's focus on contexts derived from copyrighted materials. Consider we let the model $\theta$ generate response $\boldsymbol{y}$ based on the retrieved copyrighted content $\boldsymbol{c}$ and query $\boldsymbol{x}$, then the $i$th token of the response can be sampled from the probabilistic distribution $y_i\sim p_{\theta}(y_i|\boldsymbol{c}, \boldsymbol{x}, \boldsymbol{y}_{<i})\propto\exp\mathrm{logit_{\theta}}(y_i|\boldsymbol{c}, \boldsymbol{x}, \boldsymbol{y}_{<i})$. \cad aims to remove the ``distribution'' induced by the copyrighted content, and sample $y_i$
from the distribution $y_i\sim\mathrm{softmax}[(1+\alpha)\mathrm{logit}_{\theta}(y_t|\boldsymbol{c}, \boldsymbol{x}, \boldsymbol{y}_{<i})-\alpha\mathrm{logit}_{\theta}(y_t|\boldsymbol{c}, \boldsymbol{y}_{<i})]$. $\alpha$ is the weight of adjustment and \cad is equivalent to the vanilla decoding when $\alpha=0$.




% \paragraph{Uncopy/Rewriting}


% \paragraph{Fact-Aware Retrieval Downweighting}





\subsection{Training-based Takedowns (Unlearning)}
\label{sec:unlearning_methods}

% \peter{Let's not call this training time takedown. Let's just say unlearning.}


% Machine unlearning methods attempt to remove copyrighted knowledge from a model's parameters after pretraining. We experiment with gradient ascent, gradient difference, and KL minimization approaches. 
% One typical application for machine unlearning is to mitigate the privacy risk, where we want to remove the information that the user request to be erased. Traditional machine unlearning methods includes exact unlearning, which directly retrains the model from scratch without the removed data; approximate unlearning, which modify the weights to approximate the 


Machine unlearning \citep{cao2015towards, guo2019certified}~
% \yang{@Boyi: references (especially we need to acknowledge the early works in 2019)}
is a technique designed to enable a model to ``forget'' specific information that appeared in its training data. Similarly, we can utilize unlearning as a candidate to take down copyrighted materials from the model. Most unlearning methods require a forget set (the content to be removed) and a retain set (the content to be kept). In our settings, the forget set is the copyrighted content we want to take down, and the retain set is verified licensed content from a similar distribution.
We evaluate four mainstream unlearning methods highlighted in \citet{maini2024tofu}, including: (1) \textbf{Gradient ascent}~\citep{thudi2022unrolling}, which involves maximizing the training loss for each instance in the forget set; (2) \textbf{Gradient Difference}~\citep{liu2022continual}, which increases the loss on the forget set while preserving loss on the retain set; (3) \textbf{KL minimization}~\citep{golatkar2020eternal}, which aims to minimize the KL divergence between the predictions on the retain set of the original and newly trained models while maximizing the conventional loss on the forget set; (4) \textbf{Preference Optimization}~\citep{rafailov2024direct}, which minimizes the loss of the retain set and alternative answers for the forget set. More details about the unlearning methods and dataset segmentation are available in \Cref{subsec:unlearning_details}. It's important to note that while these methods prevent the model from generating copyrighted content, they might also remove factual knowledge embedded within those copyrighted documents. 

% \weijia{@Boyi, maybe fill out extra details about the method? check the TOFU paper}\yang{We can also push these details to the appendix if we run out of space}


\iffalse
\subsection{Alignment Methods}
Unlike machine unlearning techniques, alignment methods maintain the knowledge contained within the model's parameters while ensuring that the model does not reveal copyrighted material. These methods allow the model to retain essential factual knowledge sourced from copyrighted documents without creating content that could lead to infringement. We explore preference optimization and system prompt methods.
These methods are effective \yang{are they ``effective"? maybe ``these methods are applicable to ..."} in preventing the infringement of copyrighted material embedded in the model's weights and contexts.


\paragraph{System Prompt}
The system prompt is the initial set of instructions given to an AI model that establishes the context and outlines the boundaries of its role and behavior for a specific conversation or task. This serves as a framing mechanism that guides the AI in understanding its purpose, persona, knowledge base, and the operational rules it must adhere to during interactions. We examine the impact of system prompts in preventing copyright infringement during content generation by experimenting with various options:
\weijia{Let's select one system prompt to detail here and relocate additional prompts to the appendix}
\begin{itemize}
    \item system-prompt-a \yang{Consider a more descriptive name :)}\boyi{Agreed}
    \item system-prompt-b
    \item system-prompt-c
    \item The system prompt segment from GitHub Copilot
    \item The system prompt segment from DBRX
    \item The system prompt segment from Bing Chat
\end{itemize}
\fi




% \subsection{Unlearning}
% \paragraph{Pruning with Set Difference}
% \paragraph{Gradient Ascent}
% \paragraph{Gradient Difference}
% \paragraph{KL Minimization}
% \paragraph{Preference Optimization}



==> tables/benchmark_table_deprecated.tex <==
\begin{table}[htbp]
\centering
\caption{Difference between two evaluation pipelines for NewsQA and BookSum. The main difference falls on the metrics to evaluate the utility. NewsQA uses the F1 score, while BookSum uses the ROUGE-L score.\boyi{Still need to be polished. May consider a better representation form}\weijia{@boyi give example in table or figure how does the hint and continuation looks like? }
}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{\bf Corpus} & \multicolumn{3}{c}{\bf Infringement Evaluation}    & \multicolumn{3}{c}{\bf Utility Evaluation}                                   \\ 
\cmidrule{2-7} 
                          & Exact Match               & Near Duplicate & Semantic Sim             & General & Blocklisted                      & In-Domain                   \\ 
\midrule
News                    & $\ell_\mathsf{LCS}(x,\mathcal{D}_{N\alpha})$& $\ell_\mathsf{ACS}(x,\mathcal{D}_{N\alpha})$     & $\xi(x, \mathcal{D}_{N\alpha})$                         & MMLU    & F1 for QA on $\mathcal{D}_{N\alpha}$        & F1 for QA on $\mathcal{D}_{N\beta}$        \\
\midrule
Books                   & $\ell_\mathsf{LCS}(x,\mathcal{D}_{B\alpha})$& $\ell_\mathsf{ACS}(x,\mathcal{D}_{B\alpha})$     &  $\xi(x, \mathcal{D}_{B\alpha})$                         & MMLU    & ROUGE-L for Sum on $\mathcal{D}_{B\alpha}$      & ROUGE-L for Sum on $\mathcal{D}_{B\beta}$ \\ 
\bottomrule
\end{tabular}
\label{tab:benchmark}
}
\end{table}

==> tables/results_memorization_average.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\caption{Inringement results on the memorization settings using the average value of the metics.}
\setlength{\tabcolsep}{2pt}
\begin{subtable}[t]{0.49\linewidth}
\caption{Results from news articles domain}
\resizebox{\linewidth}{!}{
\begin{tabular}{clccc}
\toprule
\multirow{2}{*}{\bf Model}              & \multirow{2}{*}{\bf Method}         & \multicolumn{3}{c}{\bf Infringement ($\downarrow$)}                    \\ 
\cmidrule{3-5} 
                                    &            & $\mathrm{mean}(\ell_\mathsf{LCS})$ &  $\mathrm{mean}(\ell_\mathsf{ACS})$ &  $\mathrm{mean}(\xi)$  \\ 
                        \midrule
\multirow{10}{*}{7B}                                             & Vanilla                          & $103.8$  & $115.5$  & $0.87$                      \\
                                                                & System Prompt                    & $1.2$ & $2.2$  & $0.23$            \\
                                                                & Gradient Ascent                  & $0.5$  & $0.5$  & $0.06$                       \\
                                                                & Gradient Difference              & $3.8$  & $3.9$  & $0.22 $                    \\
                                                                & KL Minimization                  & $0.8$ & $0.8$  &$ 0.09$                   \\
                                                                & Pref. Optimization               &$4.2$   &$19.9$   &$0.54$                \\ 
                                                                & MemFree                      & $4.6$   & $21.6$  &$0.69$                          \\
                                                                & \memfree                      & $7.7$   & $26.4$  & $0.68$                     \\
                                                                & Top-$k$ Perturbation           &$9.2_{\pm0.45}$       &$19.4_{\pm0.21}$        & $0.63_{\pm0.01}$             \\
                                                                & \cad                             &$8.7$   &$20.8$  &  $0.64$                   \\
%                         \midrule
% \multirow{2}{*}{7B-chat}                                        & Vanilla                          &$6.6$ & $13.8$ & $0.60$            \\
                                                                
                        \bottomrule
\end{tabular}}
\end{subtable}
\begin{subtable}[t]{0.49\linewidth}
\caption{Results from books domain}
\resizebox{\linewidth}{!}{
\begin{tabular}{clccc}
\toprule
\multirow{2}{*}{\bf Model}              & \multirow{2}{*}{\bf Method}         & \multicolumn{3}{c}{\bf Infringement ($\downarrow$)}                    \\ 
\cmidrule{3-5} 
                                    &            & $\mathrm{mean}(\ell_\mathsf{LCS})$ &  $\mathrm{mean}(\ell_\mathsf{ACS})$ &  $\mathrm{mean}(\xi)$  \\ 
                        \midrule
\multirow{10}{*}{7B}                                             & Vanilla                          & $106.8$  & $108.1$  & $0.99$                      \\
                                                                & System Prompt                    & $2.1$ & $2.5$  & $0.41$            \\
                                                                & Gradient Ascent                  & $3.9$  & $5.7$  & $0.45$                       \\
                                                                & Gradient Difference              & $1.7$  & $3.0$  & $0.28 $                    \\
                                                                & KL Minimization                  & $6.1$ & $9.3$  &$ 0.52$                   \\
                                                                & Pref. Optimization               &$2.4$   &$3.4$   &$0.47$                \\ 
                                                                & MemFree                      & $3.3$   & $5.1$  &$0.56$                          \\
                                                                & \memfree                      & $6.3$   & $16.6$  & $0.62$                     \\
                                                                & Top-$k$ Perturbation            &$11.8_{\pm0.99}$       &$14.0_{\pm1.06}$        & $0.61_{\pm0.01}$             \\
                                                                & \cad                             & $8.5$  & $10.5$ &  $0.62$                   \\
%                         \midrule
% \multirow{2}{*}{7B-chat}                                        & Vanilla                          &$10.2$ & $12.2$ & $0.57$            \\
                                                                
                        \bottomrule
\end{tabular}}
\end{subtable}

\label{tab:memorization_results_average}
\end{table}

==> tables/results_memorization_booksum.tex <==
\begin{subtable}[t]{\linewidth}
\caption{Results from books domain}
\resizebox{\linewidth}{!}{
\begin{tabular}{clccc|ccc|c}
\toprule
\multirow{3}{*}{\bf Model}              & \multirow{3}{*}{\bf Method}         & \multicolumn{3}{c}{\bf Infringement ($\downarrow$)}     & \multicolumn{3}{c}{\bf Utility ($\uparrow$)}           & {\bf Efficiency}               \\ 
\cmidrule{3-9} 
                                    &            & \multirow{2}{*}{$\max(\ell_\mathsf{LCS})$} &  \multirow{2}{*}{$\max(\ell_\mathsf{ACS})$} &  \multirow{2}{*}{$\max(\xi)$} &  \multirow{2}{*}{MMLU}             & Blocklisted  & In-Domain  & Inference  \\ 
                        &&&&&& ROUGE-L & ROUGE-L & Speed\\
                        \midrule
\multirow{10}{*}{7B}                                             & Vanilla                      &$150$       &$150$       &$0.96$        &$44.9$             &$11.4 $             & $11.4$                    & $1.00\times$                 \\
                                                                & System Prompt                       &$113$       &$113$       &$0.90$        & $49.4$            &  $11.8$           &  $11.4$                   & $1.00\times$                 \\
                                                                & Gradient Ascent              & $21 $     & $52$      & $0.80 $       & $40.0$           & $8.6$              & $10.1$                     & $1.00\times$                \\
                                                                & Gradient Difference          & $23$      & $76 $    & $0.86$        & $44.5$           & $9.5$              & $11.0$                     & $1.00\times$                \\
                                                                & KL Minimization              &$39$          &$76$          &$0.86$              &$44.8$                 & $10.5$                   &   $10.4$                          &$1.00\times$                    \\
                                                                & Pref. Optimization           & $26$     &$32$       & $0.76$        &$42.3$            & $1.4$              & $1.7$                     & $1.00\times$     \\
                                                                & MemFree                  & $9$         &  $24$        &   $0.77$           &$44.9$             &$11.4 $             & $11.4 $                       & $0.93\times$                   \\
                                                                & \memfree                  & $12$   &    $32$            & $0.82$              & $44.9$             &$11.4 $             & $11.4 $                       & $0.99\times$                   \\
                                                                & Top-$k$ Perturbation            &$118_{\pm16.93}$        &$135_{\pm10.21}$        & $0.93_{\pm0.01}$       &$37.7_{\pm0.91}$            &$9.5_{\pm0.23}$              &$10.2_{\pm0.29}$                      &$0.99\times$                \\
                                                                & \cad                             & $31$    & $39$      & $0.84$            & $44.9$                  &$47.5$        &$40.8$                  &$0.50\times$ \\
                                                                % & \cad                             &$31$      & $39$      &$0.84$             &$45.0$                   &$10.2$               &$9.5 $                  &$0.50\times$\\
                        % \midrule
% \multirow{2}{*}{7B-chat}                                        & Vanilla                      &$127$       &$127$       &$0.95$        & $49.1$             & $12.0$            & $11.2$                  & $1.00\times$                 \\
%                                                                 & System Prompt                      &$113$       &$113$       &$0.90$        & $49.4$            &  $11.8$           &  $11.4$                   & $1.00\times$                 \\
                        \bottomrule
                        
\end{tabular}}
\end{subtable}

==> tables/results_memorization_in_context_utility.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[ht]
\centering
\caption{Experiment results on the memorization setting, using in-context F1 score to evaluate the model's utility.}
\setlength{\tabcolsep}{2pt}
\begin{tabular}{clccc}
\toprule
\multirow{3}{*}{\bf Model}              & \multirow{3}{*}{\bf Method}         & \multicolumn{3}{c}{\bf Utility ($\uparrow$)}                    \\ 
\cmidrule{3-5} 
                                    &            & \multirow{2}{*}{MMLU} &  Blocklisted &  In-domain  \\ 
                                    &           &                      &   F1         &     F1\\
                        \midrule
\multirow{10}{*}{7B}                                             & Vanilla                          & $45.0$  & $63.2$  & $31.1$                      \\
                                                                & Gradient Ascent                  & $44.2$  & $10.2$  & $6.7$                       \\
                                                                & Gradient Difference              & $44.3$  & $26.1$  & $33.9$                    \\
                                                                & KL Minimization                  & $44.2$ & $12.2$  &$ 9.3$                   \\
                                                                & Pref. Optimization               &$38.6$   &$37.6$   &$45.8$                \\ 
                                                                & MemFree                      & $45.0$  & $63.2$  & $31.1$                          \\
                                                                & \memfree                      & $45.0$  & $63.2$  & $31.1$                    \\
                                                                & Top-$k$ Perturbation           &$40.3_{\pm1.10}$       &$20.5_{\pm1.51}$        & $20.2_{\pm0.97}$             \\
                                                                & \cad                             &$45.0$   &$39.3$  &  $42.1$                   \\
%                         \midrule
% \multirow{2}{*}{7B-chat}                                        & Vanilla                          &$10.2$ & $12.2$ & $0.57$            \\
                                                                
                        \bottomrule
\end{tabular}

\label{tab:memorization_results_in_context_qa}
\end{table}

==> tables/results_rag_average.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\caption{Inringement results for RAG setting using the average value of the metrics.}
\setlength{\tabcolsep}{2pt}
\begin{subtable}[t]{0.495\linewidth}
\caption{Results on news articles domain}
\resizebox{\linewidth}{!}{
\begin{tabular}{clccc}
\toprule
\multirow{2}{*}{\bf Model} & \multirow{2}{*}{\bf Method}         & \multicolumn{3}{c}{\bf Infringement ($\downarrow$)}                 \\ 
\cmidrule{3-5} 
                            &             & $\mathrm{mean}(\ell_\mathsf{LCS})$ &  $\mathrm{mean}(\ell_\mathsf{ACS})$ &  $\mathrm{mean}(\xi)$ \\
                        \midrule
\multirow{5}{*}{7B-Chat}                                        & Vanilla                          & $14.4$  & $22.2$  & $0.65$         \\ %68.24
                                                                & System prompt                    & $4.6$  & $7.1 $ & $0.48$              \\ % 384
                                                                & Top-$k$ Perturbation                &$4.7_{\pm0.80}$   &$8.9_{\pm1.3}$   &$0.62_{\pm0.02}$ \\ % 365
                                                                & MemFree                        & $2.2$    & $8.4$  & $0.60$                    \\
                                                                & \memfree                   & $2.6$    & $6.4$  &   $0.58$                  \\ 
                        \midrule
\multirow{5}{*}{70B-Chat}                                        & Vanilla                            &$67.0$   &$90.8$  &$0.84$         \\%63.7
                                                                & System prompt                    &$39.0$   &$70.4$   &$0.82$            \\ % 64.8
                                                               & Top-$k$ Perturbation                &$18.7_{\pm2.23}$   &$34.2_{\pm2.54}$   &  $0.71_{\pm0.01}$    \\ % 62.9
                                                               & MemFree          & $4.8$   & $45.7$  &   $0.77$                            \\
                                                               & \memfree        & $6.3$   & $22.2$  &   $0.65$         \\ % 62.9
                        \bottomrule
\end{tabular}}
\end{subtable}
\begin{subtable}[t]{0.495\linewidth}
\caption{Results on books domain}
\resizebox{\linewidth}{!}{
\begin{tabular}{clccc}
\toprule
\multirow{2}{*}{\bf Model} & \multirow{2}{*}{\bf Method}         & \multicolumn{3}{c}{\bf Infringement ($\downarrow$)}                 \\ 
\cmidrule{3-5} 
                            &             & $\mathrm{mean}(\ell_\mathsf{LCS})$ &  $\mathrm{mean}(\ell_\mathsf{ACS})$ &  $\mathrm{mean}(\xi)$ \\
                        \midrule
\multirow{5}{*}{7B-Chat}                                        & Vanilla                          & $58.5$  & $69.2$  & $0.77$         \\ %68.24
                                                                & System prompt                    & $31.3$  & $34.2 $ & $0.55$              \\ % 384
                                                                & Top-$k$ Perturbation                &$9.5_{\pm1.37}$   &$14.5_{\pm1.53}$   &$0.58_{\pm0.01}$ \\ % 365
                                                                & MemFree                        & $3.5$    & $14.6$  & $0.58$                    \\
                                                                & \memfree                   & $4.3$    & $12.4$  &   $0.59$                  \\ 
                        \midrule
\multirow{5}{*}{70B-Chat}                                        & Vanilla                            & $84.1$  & $93.5$  & $0.81$         \\%63.7
                                                                & System prompt                    &$71.3$   &$86.6$   &$0.81$            \\ % 64.8
                                                               & Top-$k$ Perturbation              &$20.8_{\pm0.69}$   &$38.5_{\pm2.12}$   &  $0.70_{\pm0.02}$        \\ % 62.9
                                                               & MemFree          & $6.4$   & $50.3$  & $0.96$                              \\
                                                               & \memfree        & $6.6$   & $27.2$  &   $0.96$         \\ % 62.9
                        \bottomrule
\end{tabular}}
\end{subtable}


\label{tab:rag_results_average}
\end{table}

==> tables/system_prompt_ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\caption{Ablation study on the impact of sensitive keywords (``CNN'' in our experiment) on the system prompt's final performance. Removing the sensitive keywords diminishes the effect of the system prompt.}
\centering
\resizebox{\linewidth}{!}{
\setlength{\tabcolsep}{2pt}
\begin{tabular}{clcccccc}
\toprule
\multirow{2}{*}{\bf Model}              & \multirow{2}{*}{\bf Method}         & \multicolumn{6}{c}{\bf Infringement ($\downarrow$)}                    \\ 
\cmidrule{3-8} 
                                    &            & $\max(\ell_\mathsf{LCS})$ &  $\max(\ell_\mathsf{ACS})$ &  $\max(\xi)$ & $\mathrm{mean}(\ell_\mathsf{LCS})$ &  $\mathrm{mean}(\ell_\mathsf{ACS})$ &  $\mathrm{mean}(\xi)$  \\ 
                        \midrule
\multirow{4}{*}{7B-Chat}                                            & Vanilla                            &$127$       &$127$       &$0.95$    &$6.6$ & $13.8$ & $0.60$                   \\
                                                                & Vanilla (No ``CNN'')                          & $78$  & $83$  & $0.96$     & $5.4$ & $10.5$ & $0.59$                  \\       
                                                                & System Prompt                    & $11$ & $37$  & $0.83$        & $1.2$ & $2.2$  & $0.23$    \\
                                                                & System Prompt (No ``CNN'')                   & $20$ & $44$  & $0.84$         & $1.2$ & $2.4$  & $0.25$    \\

%                         \midrule
% \multirow{2}{*}{7B-chat}                                        & Vanilla                          &$10.2$ & $12.2$ & $0.57$            \\
                                                                
                        \bottomrule
\end{tabular}}

\label{tab:sys_prompt_ablation}
\end{table}
